Robust Filtering -- Novel Statistical Learning and Inference Algorithms with Applications

State estimation or filtering serves as a fundamental task to enable intelligent decision-making in applications such as autonomous vehicles, robotics, healthcare monitoring, smart grids, intelligent transportation, and predictive maintenance. Standard filtering assumes prior knowledge of noise statistics to extract latent system states from noisy sensor data. However, real-world scenarios involve abnormalities like outliers, biases, drifts, and missing observations with unknown or partially known statistics, limiting conventional approaches. This thesis presents novel robust nonlinear filtering methods to mitigate these challenges. Based on insights from our filtering proposals, we extend the formulations to offline estimation/learning setups and propose smoothing extensions. Our methods leverage Bayesian inference frameworks, employing both deterministic and stochastic approximation techniques including Variational Inference (VI) and Particle Filters/Sequential Monte Carlo (SMC). We also study theoretical estimation limits using Bayesian Cram\'er-Rao bounds (BCRBs) in the context of measurement abnormalities. To validate the performance gains of the proposed methods, we perform simulations and experiments in scenarios including target tracking, indoor localization, 3D point cloud registration, mesh registration, and pose graph optimization. The fundamental nature of the work makes it useful in diverse applications, with possible future extensions toward developing outlier-robust machine learning pipelines, learning system dynamics from anomalous data, and addressing challenges in generative AI where standard diffusion models struggle with outliers, imbalanced datasets, and mode collapse.

==> MainText/publications.tex <==
\addtocontents{toc}{\vspace{2em}} % Add a gap in the Contents, for aesthetics
\unnumberedchapter{Published articles} % Title of the unnumbered chapter
\chapter*{Published articles} % Starts a chapter which will remain empty

For convenience of the examiners, you may include here any number of PDF documents such as papers you published or submitted. Those documents will appear in the temporary version of the thesis, but will not be rendered on the final version to avoid copyright issues.

\includepdf[pages=-, offset=0.54cm \voffset]{./Images/papers/ch01_who-we-are_en_20151028_cl.pdf} % Includes pdf
%\includepdf[pages=-, offset=0.54cm \voffset]{./Images/papers/paper2.pdf} % Includes pdf
%\includepdf[pages=-, offset=0.54cm \voffset]{./Images/papers/paper3.pdf} % Includes pdf
